A Brief History of Prompt: Leveraging Language Models. (Through Advanced Prompting)

This paper presents a comprehensive exploration of the evolution of prompt engineering and generation in the field of natural language processing (NLP). Starting from the early language models and information retrieval systems, we trace the key developments that have shaped prompt engineering over the years. The introduction of attention mechanisms in 2015 revolutionized language understanding, leading to advancements in controllability and context-awareness. Subsequent breakthroughs in reinforcement learning techniques further enhanced prompt engineering, addressing issues like exposure bias and biases in generated text. We examine the significant contributions in 2018 and 2019, focusing on fine-tuning strategies, control codes, and template-based generation. The paper also discusses the growing importance of fairness, human-AI collaboration, and low-resource adaptation. In 2020 and 2021, contextual prompting and transfer learning gained prominence, while 2022 and 2023 witnessed the emergence of advanced techniques like unsupervised pre-training and novel reward shaping. Throughout the paper, we reference specific research studies that exemplify the impact of various developments on prompt engineering. The journey of prompt engineering continues, with ethical considerations being paramount for the responsible and inclusive future of AI systems.

==> tables-figures/crosswalk-area-definition.tex <==
\begin{figure}[bt!]
    \begin{subfigure}[b]{.5\linewidth}
      \centering
      \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-1.PNG}}
      \caption{}
      \label{fig:crosswalk-area-definition-a}
    \end{subfigure}%%
    \begin{subfigure}[b]{.5\linewidth}
      \centering
      \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-midblock.PNG}}
      \caption{}
      \label{fig:crosswalk-area-definition-b}
    \end{subfigure}
    \caption{The pedestrian is crossing from the South towards the North. (a) The effective area around a designed crosswalk. (b) The effective area with respect to the source position of the pedestrian for mid-block crossing.}
    \label{fig:crosswalk-area-definition}
\end{figure}

==> templates/1-figure.tex <==
\begin{figure}[bt!]

    \centering
    \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-1.PNG}}
    \caption{(a) K-shaped with one road having median restricted lanes (right bottom), (b) long-connections, (c) single outgoing lane road in a 3-way intersection.}
    \label{fig:2-sub-figure}
\end{figure}

==> templates/2-sub-figure.tex <==
\begin{figure}[bt!]
    \begin{subfigure}[b]{.5\linewidth}
      \centering
      \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-1.PNG}}
      \caption{}
      \label{fig:4-way-k}
    \end{subfigure}%%
    \begin{subfigure}[b]{.5\linewidth}
      \centering
      \framebox{\includegraphics[width=.9\linewidth]{images/crosswalk-area-midblock.PNG}}
      \caption{}
    \end{subfigure}
    \caption{(a) K-shaped with one road having median restricted lanes (right bottom), (b) long-connections, (c) single outgoing lane road in a 3-way intersection.}
    \label{fig:2-sub-figure}
\end{figure}

==> templates/table.tex <==
Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

